On Evaluating Explanation Utility for Human-AI Decision Making in NLP

Is explainability a false promise? This debate has emerged from the insufficient evidence that explanations help people in situations they are introduced for. More human-centered, application-grounded evaluations of explanations are needed to settle this. Yet, with no established guidelines for such studies in NLP, researchers accustomed to standardized proxy evaluations must discover appropriate measurements, tasks, datasets, and sensible models for human-AI teams in their studies. To aid with this, we first review existing metrics suitable for application-grounded evaluation. We then establish criteria to select appropriate datasets, and using them, we find that only 4 out of over 50 datasets available for explainability research in NLP meet them. We then demonstrate the importance of reassessing the state of the art to form and study human-AI teams: teaming people with models for certain tasks might only now start to make sense, and for others, it remains unsound. Finally, we present the exemplar studies of human-AI decision-making for one of the identified tasks -- verifying the correctness of a legal claim given a contract. Our results show that providing AI predictions, with or without explanations, does not cause decision makers to speed up their work without compromising performance. We argue for revisiting the setup of human-AI teams and improving automatic deferral of instances to AI, where explanations could play a useful role.

==> tables/base_ex_ds42.tex <==

\begin{table*}[h]\centering
\small
\begin{tabular}{p{15cm}p{0.01cm}}\toprule
Determine if the claim is true based on the text below:\textbackslash n Claim: Mitt Romney said he thinks airplane windows should be able to roll down in case of fire.\textbackslash n\textbackslash nOptions: True, False, Not enough information\textbackslash n\textbackslash n1.\textbackslash n-Mitt Romney, in leaked comments from a fundraiser in May 2012 2.
\textbackslash n\quotes{When you have a fire in an aircraft, there's no place to go, exactly, there's no -- and you can't find any oxygen from outside the aircraft to get in the aircraft, because the windows don't open.
\textbackslash nI don't know why they don't do that.}\textbackslash n-Mitt Romney, suggesting it would be a good idea to crack a window at 35,000 feet, Beverly Hills fundraiser, Sept. 22, 2012 4.\textbackslash n-Mitt Romney (January 2012) 6.
\textbackslash n-Mitt Romney, in leaked comments from a Florida fundraiser, May 17 2012 9.
\textbackslash n\quotes{Actually, I didn't say that.}\textbackslash n-Mitt Romney, committing a gaffe while introducing his running mate, Norfolk, Va., Aug. 11, 2012 \quotes{I should tell my story.}\textbackslash n-Mitt Romney, speaking in 2011 to unemployed people in Florida.
\textbackslash n-Mitt Romney (May 17, 2012)\textbackslash nJust chatted w/Mitt Romney at Logan Airport in the security line, what a humble, friendly gentleman.\textbackslash nShook hands and spoke with Mitt Romney at Salt Lake Airport.\textbackslash nMitt Romney is a mouth breather, based on this creepy picture my sister just sent me from her plane.
\textbackslash nJust sat next to @MittRomney on my flight to SLC.\textbackslash nJust sat next to @MittRomney on my flight to SLC.
\textbackslash nSat next to nice guy @MittRomney on way to \#NGIMeetUp Enjoyed discussion and he even had the middle seat in coach Sat next to nice guy @MittRomney on way to \#NGIMeetUp Enjoyed discussion and he even had the middle seat in coach And in coach, what are the odds!
\textbackslash nThanks @MittRomney for taking a picture with us!\textbackslash n\#saltlakeairport \#usubasketball Thanks @MittRomney for taking a picture with us!
\textbackslash nWith little fanfare for the much-expected move, the former Massachusetts governor revealed the decision in an understated video posted on a website and on his Facebook page.
\textbackslash nRomney then put out a Twitter message at 3:43 p.m. and directed supporters to www.mittromney.com , which included the video.\textbackslash nWithin hours, Democrats nationally began criticizing Romney.\textbackslash nIt is a sacrifice the Republican presidential candidate did not make.\textbackslash nHis campaign has refused to comment publicly on the subject over the past week.\textbackslash nRock said in the 2008 interview.\textbackslash nIt was all in good fun.\textbackslash nEven though this latest statement by Mitt Romney will undoubtedly be spun so that it will be seen as being taken out of context, someone needs to tell this man to just keep his mouth shut and smile.\textbackslash nThe Romney campaign has yet to release its version of the speech made in Prattville.\textbackslash nObama went along with this outlandish bunkum until recently when he delayed another new air regulation until 2013.\textbackslash nThen there's former Governor Mitt Romney.\textbackslash nIt was all in good fun.\textbackslash nIt is not known if the former Governor has heard this quote yet.
\textbackslash n				 \\
\bottomrule
\end{tabular}
\caption{A representative input sample for the Snopes task. The template is: Determine if the claim is true based on the text below:\textbackslash n Claim: {\textbf{claim}}\textbackslash n\textbackslash \textbf{nOptions}: True, False, Not enough information\textbackslash n\textbackslash n{\textbf{text}}\textbackslash n{answer}: }
\label{tab:snopes_example}
\end{table*}


==> tables/results_all.tex <==
\begin{table*}[t]
    \centering
    \begin{adjustbox}{valign=t}
    \begin{subtable}[t]{.35\linewidth}
        \centering
        \resizebox{\linewidth}{!}{
        \begin{tabular}{lccc}\toprule
        &\textbf{P} &\textbf{R} &\textbf{F1}\\\midrule
        \multicolumn{4}{l}{\textbf{Flan-T5-3B (our)}} \\
        \arrayrulecolor{black!20}\midrule
        \textsc{Entail} &92.5 &93.7 &93.1 \\
        \textsc{No Mention} &93.0 &87.0 &89.9 \\
        \textsc{Contradict} &68.7 &82.7 &75.0 \\
        \arrayrulecolor{black!20}\midrule
        \textsc{Micro Avg.} &90.2 &89.7 &89.8 \\
        \textsc{Macro Avg.} & 84.7 & 87.7 & 86.0 \\
        \textsc{Macro (E,C)} & 80.6 & 88.2 & \textbf{84.1} \\
        \arrayrulecolor{black}\midrule
        \multicolumn{4}{l}{\textbf{BERT-Large} }\\ %
        \arrayrulecolor{black!20}\midrule
        \textsc{Entail} &- &- &83.4  \\
        \multicolumn{4}{l}{\textsc{No mention} (\emph{not reported}) }\\
        \textsc{Contradict} &- &- &35.7 \\
        \arrayrulecolor{black!20}\midrule
        \textsc{Macro (E,C)} & - & - & 59.6 \\
        \arrayrulecolor{black}\bottomrule
        \end{tabular}
        }
        \caption{ContractNLI}
        \label{tab:contractnli_results_all}
    \end{subtable}%
    \end{adjustbox}
    \begin{adjustbox}{valign=t}
    \begin{subtable}[t]{.35\linewidth}
        \centering
        \resizebox{\linewidth}{!}{
        \begin{tabular}{lccc}\toprule
        &\textbf{P} &\textbf{R} &\textbf{F1}\\\midrule
        \multicolumn{4}{l}{\textbf{Flan-T5-3B (our)}} \\
        \arrayrulecolor{black!20}\midrule
        \textsc{Increase}        &52.7	    &64.4	     &58.8 \\
        \textsc{No Diff}         &54.7	    &29.2	     &38.1 \\
        \textsc{Decrease}        &41.1	    &59.1	    &48.5 \\
        \arrayrulecolor{black!20}\midrule
        \textsc{Micro Avg.}      &50.7	    &49.1	     &47.6 \\
        \textsc{Macro Avg.}      &49.5	    &51.6	     & 48.5 \\
        \arrayrulecolor{black}\midrule
        \multicolumn{4}{l}{\textbf{NN + pretrain cond. attn.} } \\ %
        \arrayrulecolor{black!20}\midrule
        \textsc{Macro Avg.}       &53.0    &51.8    &52.1 \\
        \arrayrulecolor{black}\bottomrule
        \end{tabular}
        }
        \caption{EvidenceInference v2 with retrieval}
        \label{tab:ild_results_all}
    \end{subtable}%
    \end{adjustbox}
    \caption{Finetuned Flan-T5-3B and the state-of-the-art reported results. XLNet+BiGRU \citep{malik-etal-2021-ildc}; Neural network + Pretrain conditional attention \citep{lehman-etal-2019-inferring} ;
    MultiVerS \citep{wadden-etal-2022-multivers}; BERT-Large  \citep{koreeda-manning-2021-contractnli-dataset}. \citet{wadden-etal-2022-multivers} estimate the human performance in the ``abstract-provided'' setting.}
    \label{tab:all_results}
\end{table*}



